Sequential Fair Allocation: Achieving the Optimal Envy-Efficiency Tradeoff Curve

We consider the problem of dividing limited resources to individuals arriving over $T$ rounds. Each round has a random number of individuals arrive, and individuals can be characterized by their type (i.e. preferences over the different resources). A standard notion of 'fairness' in this setting is that an allocation simultaneously satisfy envy-freeness and efficiency. The former is an individual guarantee, requiring that each agent prefers their own allocation over the allocation of any other; in contrast, efficiency is a global property, requiring that the allocations clear the available resources. For divisible resources, when the number of individuals of each type are known upfront, the above desiderata are simultaneously achievable for a large class of utility functions. However, in an online setting when the number of individuals of each type are only revealed round by round, no policy can guarantee these desiderata simultaneously, and hence the best one can do is to try and allocate so as to approximately satisfy the two properties. We show that in the online setting, the two desired properties (envy-freeness and efficiency) are in direct contention, in that any algorithm achieving additive counterfactual envy-freeness up to a factor of $L_T$ necessarily suffers a efficiency loss of at least $1 / L_T$. We complement this uncertainty principle with a simple algorithm, HopeGuardrail, which allocates resources based on an adaptive threshold policy and is able to achieve any fairness-efficiency point on this frontier. In simulation results, our algorithm provides allocations close to the optimal fair solution in hindsight, motivating its use in practical applications as the algorithm is able to adapt to any desired fairness efficiency trade-off.

==> parts/alg_pseudocode.tex <==
\section{Pseudocode for \HopeGuardrail}
\label{sec:pseudocode}

\begin{algorithm}[!h]
\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
\KwIn{Budget $B$, $(\Exp{N_{\theta}})_{\theta \in \Theta}$, confidence terms $(\conf_{t, \theta})_{\theta \in \Theta}$, and a desired bound on envy $L_T$}
\KwOut{An allocation $X^{alg} \in \mathbb{R}^{T \times |\Theta| \times K}$}
Set $\multconf_{t} = \max_{\theta} \frac{\conf_{t, \theta}}{\Exp{N_{\geq t, \theta}}}$ for all $t \leq T$;

Solve for $\overline{X} = x(\underline{n}_{\theta})$ as the solution to \cref{eq:eg} where $\underline{n}_{\theta} = \Exp{N_{\theta}}(1 - \multconf_1)$ \tcp*[h]{solve for our optimistic and pessimistic guardrails}\;
Solve for $\underline{X} = x(\overline{n}_{\theta})$ as the solution to \cref{eq:eg} where $\overline{n}_{\theta} = \Exp{N_{\theta}}(1 + \multconf_1)$. \;
\For{rounds $t = 1, \ldots, T-\Ts$}{ 
    \For{each resource $k \in [K]$}{
    \uIf(\tcp*[h]{insufficient budget to allocate lower threshold}){$B_{t,k}^{alg} < \sum_{\theta \in \Theta} N_{t, \theta} \underline{X}_{\theta, k}$}{
        Set $X_{t, \theta, k}^{alg} = \frac{B_{t,k}^{alg}}{\sum_{\theta \in \Theta} N_{t, \theta}}$ for each $\theta \in \Theta$\;}
    \uElseIf(\tcp*[h]{\cyedit{use upper allocation}}){$B_{t,k}^{alg} - \sum_{\theta} N_{t, \theta} \overline{X}_{\theta, k} \geq \sum_{\theta \in \Theta} \underline{X}_{\theta, k} (\Exp{N_{> t, \theta}} + \conf_{t, \theta})$}{
        Set $X_{t, \theta, k}^{alg} = \overline{X}_{\theta, k}$ for each $\theta \in \Theta$\;}
    \uElse(\tcp*[h]{\cyedit{use lower allocation}}){
        Set $X_{t, \theta, k}^{alg} = \underline{X}_{\theta, k}$ for each $\theta \in \Theta$\;}
    }
        Update $B_{t+1}^{alg} = B_t^{alg} - \sum_{\theta \in \Theta} N_{t, \theta} X_{t, \theta}^{alg}$
}
% \For(\tcp*[h]{switch to conservative rule}){remaining rounds $t=\Ts+1,\Ts+2,\ldots,T$}{ 
% Set $X_{t, \theta}^{alg} = \min\left\{\underline{X}_{\theta},\frac{B_t^{alg}}{\sum_{\theta \in \Theta} N_{t, \theta}}\right\}$ for each $\theta \in \Theta$\;
% Update $B_{t+1}^{alg} = B_t^{alg} - \sum_{\theta \in \Theta} N_{t, \theta} X_{t, \theta}^{alg}$ \;
% }
\Return{$X^{alg}$}
	\caption{Histogram of Preference Estimates with Guardrails (\HopeGuardrail)}
	\label{alg:brief}
\end{algorithm}

==> parts/relation_guarantees.tex <==
\subsection{Relationship between Approximate Envy and Efficiency to Varian Fairness}
\label{app:relation_fairness}

Here we briefly relate the definitions from \cref{def:distance} to online counterparts to \cref{def:fairness}.  We start by repeating \cref{def:distance} for clarity.

\begin{definition}[Fair Allocation (\cref{def:distance})]
Given types $(\theta)_{\theta \in \Theta}$, the number of individuals of each type $(N_{t, \theta})_{t \in [T], \theta \in \Theta}$ and utility functions $(u(\cdot,\theta))_{\theta \in \Theta}$, an allocation $X = \{X_{t, \theta}\in\mathbb{R}^K_+ \mid \sum_{t=1}^T \sum_{\theta \in \Theta} N_{t, \theta} X_{t, \theta} \leq B\}$ is said to be fair if it simultaneously satisfies the following:
\begin{enumerate}
\item \textit{Envy-Freeness} (EF): For every pair of rounds $t,t'$ and types $\theta, \theta'$, we have $u(X_{t, \theta}, \theta) \geq u(X_{t', \theta'}, \theta)$.
\item \textit{Pareto-Efficiency} (PE): For any allocation ${Y}\neq X$ such that $u(Y_{t, \theta},\theta)> u(X_{t, \theta},\theta)$ for some round $t$ and type $\theta$, there exists some other round $t'$ and type $\theta'$ such that $u(Y_{t', \theta'},\theta')< u(X_{t', \theta'}, \theta')$. 
\item \textit{Proportional} (Prop): For any round $t$, type $\theta$ we have $u(X_{t, \theta}, \theta) \geq u(B/N, \theta)$ where $N = \sum_{t=1}^T \sum_{\theta \in \Theta} N_{t, \theta}$.
\end{enumerate}
\end{definition}


